The new $(g-2)_\mu$ and Right-Handed Sneutrino Dark Matter

In this paper we investigate the $(g-2)_\mu$ discrepancy in the context of the R-parity conserving next-to-minimal supersymmetric Standard Model plus right-handed neutrinos superfields. The model has the ability to reproduce neutrino physics data and includes the interesting possibility to have the right-handed sneutrino as the lightest supersymmetric particle and a viable dark matter candidate. Since right-handed sneutrinos are singlets, no new contributions for $\delta a_{\mu}$ with respect to the MSSM and NMSSM are present. However, the possibility to have the right-handed sneutrino as the lightest supersymmetric particle opens new ways to escape Large Hadron Collider and direct detection constraints. In particular, we find that dark matter masses within $10 \lesssim m_{\tilde{\nu}_{R}} \lesssim 600$ GeV are fully compatible with current experimental constraints. Remarkably, not only spectra with light sleptons are needed, but we obtain solutions with $m_{\tilde{\mu}} \gtrsim 600$ GeV in the entire dark matter mass range that could be probed by new $(g-2)_\mu$ data in the near future. In addition, dark matter direct detection experiments will be able to explore a sizable portion of the allowed parameter space with $m_{\tilde{\nu}_{R}} \lesssim 300$ GeV, while indirect detection experiments will be able to probe a much smaller fraction within $200 \lesssim m_{\tilde{\nu}_{R}} \lesssim 350$ GeV.

==> defsV3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%                 Last Version 2019                    %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%                    begin macros                     %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[T1]{fontenc}
\usepackage{epsfig}
\usepackage{latexsym}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsfonts}   % if you want the fonts
\usepackage{amssymb}    % if you want extra symbols
\usepackage{float}
\usepackage{bm}
%\usepackage{cite}
\usepackage{url}
\usepackage{hyperref} 
\usepackage[nodisplayskipstretch]{setspace}
\setstretch{1.0}
%\usepackage{subfig}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator{\sgn}{sgn}
\def\tcb{\textcolor{blue}} 
\def\met{\ensuremath{E_{\mathrm{T}}^{\mathrm{miss}}}}
\def\amass{m_A^2}
\def\higgsu{m_{H_u}^2}
\def\higgsd{m_{H_d}^2}
\def\higgsuew{m_{H_u}^2(M_Z)}
\def\higgsdew{m_{H_d}^2(M_Z)}
\def\H{H^0}
\def\h{h^0}
\def\msq{m_{Q_3}^2}
\def\msu{m_{u_3}^2}
\def\msd{m_{d_3}^2}
\def\msl{m_{L_3}^2}
\def\mse{m_{e_3}^2}
\def\neumass{m_{\tilde\chi_1^0}}
\newcommand{\crosssec}{\sigma_{\tilde\chi^0_1-p}}
\def\tanb{\tan\beta}
\def\tgb{\tan\beta}
\def\neut{\tilde\chi_1^0}
\def\bsg{$b\to s\gamma$}
\def\stau{\tilde\tau_1}
\def\asusy{a^{\rm SUSY}_\mu}
\def\resonance{$m_{A^0}\approx2\neumass$}
\def\k{\kappa}
\def\l{\lambda}
\def\ee{e^+e^-\to h^0Z}
\def\VMnote#1{{\bf[VM: #1]}}
\def\Rnote#1{{\bf[RR: #1]}}
\def\Lnote#1{{\bf[DL: #1]}}
\def\Mnote#1{{\bf[CM: #1]}}
\def\Gnote#1{{\bf[PG: #1]}}
\def\ck{{\bf[Check!]}}
\def\lsim{\raise0.3ex\hbox{$\;<$\kern-0.75em\raise-1.1ex\hbox{$\sim\;$}}}
\def\gsim{\raise0.3ex\hbox{$\;>$\kern-0.75em\raise-1.1ex\hbox{$\sim\;$}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% def (Cyril)
\def\nmh{{\sc nmhdecay}}
\newcommand{\captions}{\sf\caption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  def (Daniel)
\def    \beq            {\begin{equation}}
\def    \eeq            {\end{equation}}
\def    \bea           {\begin{eqnarray}}
\def    \eea           {\end{eqnarray}}
\def    \nn            {\nonumber}
\def  \dsum   { \mathbf{\sum} }
\def \dprod   {\mathbf{\prod}}
\def \dint   {\mathbf{\int}}
\def \doint   {\mathbf{\oint}}
\def \tprod   {{\tiny \mathbf{\prod}}}
\def \ie{{\it i.e.}}
\def \eg{{\it e.g.}}
\def \etal{{\it et al.}}
\def \snuc{\tilde{\nu}^c}
\def \snu{\tilde{\nu}}
\def \mn{\mu\nu{\rm SSM}}
\def\n{\widetilde\chi^0}
\def\c{\widetilde\chi^\pm}
\def\bl{\bm\lambda}
\def\w{W^\pm}
\def\S{S^0}
\def\P{P^0}
\def\g2{{\rm GeV}^2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    def (Roberto)
\def\tb{{\rm tan}\beta}
\def\sb{{\rm sin}\beta}
\def\cb{{\rm cos}\beta}
\def\mht{m^{\rm tree}_h}
\def\vi{\nu_i}
\def\vci{\nu^c_i}
\def\n{\widetilde\chi^0}
\def\nc{\nu^c}
\def\vd{v_d}
\def\vu{v_u}
\def\mHd{m_{H_d}}
\def\mHu{m_{H_u}}
\def\mL{m_{\tilde L}}
\def\mNU{m_{\tilde{\nu}^c}}
\def\sw2{sin^2 \theta_w}
\def\drbar{\overline{DR}}
\def\msbar{\overline{MS}}
\def\diag{\mathrm{diag}}
\def\I{\mathrm{i}}
\def\at{\alpha_t}
\def\ab{\alpha_b}
\def\as{\alpha_s}
\def\a^tau{\alpha_{\tau}}
\def\oat{{\cal O}(\at)}
\def\oab{{\cal O}(\ab)}
\def\oatau{{\cal O}(\atau)}
\def\oatab{{\cal O}(\at\ab)}
\def\oatas{{\cal O}(\at\as)}
\def\oabas{{\cal O}(\ab\as)}
\def\oatababq{{\cal O}(\at\ab + \ab^2)}
\def\oatqatababq{{\cal O}(\at^2 + \at\ab + \ab^2)}
\def\oatasatq{{\cal O}(\at\as + \at^2)}
\def\oatasabas{{\cal O}(\at\as +\ab\as)}
\def\oatasabasatq{{\cal O}(\at\as + \at^2 +\ab\as)}
\def\oatq{{\cal O}(\at^2)}
\def\oabq{{\cal O}(\ab^2)}
\def\oatauq{{\cal O}(\atau^2)}
\def\oabatau{{\cal O}(\ab \atau)}
\def\oas{{\cal O}(\as)}
\def\oatauqatab{{\cal O}(\atau^2 +\ab \atau )}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\beqa{\begin{eqnarray}}
\def\eeqa{\end{eqnarray}}
\def\vb#1{\vbox to #1 pt{}}
\def\smallfrac#1#2{{\textstyle{#1 \over #2}}}
\def\rpb{R_p \hspace{-0.155in} \slash}
\newcommand{\vev}{\textrm{VEV}}
\newcommand{\vevs}{\textrm{VEVs}}
\newcommand{\tev}{\,\textrm{TeV}}
\newcommand{\gev}{\,\textrm{GeV}}
\newcommand{\mev}{\,\textrm{MeV}}
\newcommand{\kev}{\,\textrm{keV}}
\newcommand{\ev}{\,\textrm{eV}}
\newcommand{\eV}{\,\textrm{eV}}
\newcommand{\km}{\,\textrm{km}}
\newcommand{\cm}{\,\textrm{cm}}
\newcommand{\fm}{\,\textrm{fm}}
\newcommand{\pb}{\,\textrm{pb}}
\newcommand{\fb}{\,\textrm{fb}}
\newcommand{\del}[1]{ {\bf DL: #1 } }
\newcommand{\Mp}{M_P}
\newcommand{\gravitino}{{\tilde{G}}}
\newcommand{\mgravitino}{{m_{\tilde{G}}}}
\newcommand{\neutralino}{{\tilde{\chi}^0}}
\newcommand{\mneutralino}{{m_{\tilde{\chi}^0}}}
\newcommand{\bfrac}[2]{{\left(\frac{#1}{#2} \right)  }}
%%%%%%%%%%%%%%%%%%%%%% end macros %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% begin flavor variables and decays            %%%%%%%
% \def\bsgam{$b\rightarrow s\gamma$ }
\newcommand{\newc}{\newcommand}
\newc\BR{BR}
\newc{\akappa}{A_{\kappa} }
\newc\deltagmtwo{\delta (g-2)_{\mu}} 
\newc\deltaamu{\Delta a_{\mu}}
\def\caibb{C_{\ai b\anti b}}
\def\br{BR}
\def\anti{\overline}
\def\ai{a_1}
\def\wt{\widetilde}
%\def\MET{E_T \hspace{-1.2em}/\;\:}
%\def\rpv{R_p \hspace{-1.2em}/\;\:}
\def\fbi{\rm fb^{-1}}
\def\rf{{\bf{[ref] }}}
\def\la{\lambda}
\def\bla{\bm \lambda}
\def\ka{\kappa}
\def\Ala{A_\lambda}
\def\Aka{A_\kappa}
%\def\rpv{\not\!\!{R_p}}
\def\rpv{{R}_{p} \hspace{-0.4cm}\slash\hspace{0.2cm}}
\def\MET{{E}_{\rm T} \hspace{-0.43cm}\slash\hspace{0.2cm}}
\newc{\haa}{BR\(h_1\to a_1 a_1\)}
\newc{\abb}{BR\(a_1\to b\anti{b}\)}
\newc{\hbb}{BR\(h_1\to b\anti{b}\)}
\newc{\abund}{\Omega h^2}
\newc\bsgamma{b\rightarrow s \gamma }
\newc\bxsgamma{\overline{B}\rightarrow X_{s}\gamma}
\newc\brbsgamma{\BR(\overline{B}\rightarrow X_s\gamma)}
\newcommand\bsmumu{\overline{B}_s\to\mu^+\mu^-}
\newcommand\brbsmumu{\BR(\overline{B}_s\to\mu^+\mu^-)}
\newcommand\bdmmumu{\overline{B}_d\to\mu^+\mu^-}
\newcommand\bbbarmix{\overline{B}_s\mbox{-}B_s}      % B_s mixing
% \newcommand\bbbarmix{\bar{B}_s-B_s}      % B_s mixing
\newcommand\delmbs{\Delta M_{B_s}}
\newcommand\brbtaunu{\BR(\overline{B}_u\to \tau \nu)}
%%%%%% end flavor variables and decays            %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% def (Pradipta)
%\tolerance = 50000
%\textwidth 6.5in 
%\textheight 9.8in %       25cm
%\topmargin -0.7in
%\topmargin -0.4in
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Def German
\newc{\Fermi}{\textit{Fermi}-}

%%%%
